Continuous DR-submodular Maximization: Structure and Algorithms

DR-submodular continuous functions are important objectives with wide real-world applications spanning MAP inference in determinantal point processes (DPPs), and mean-field inference for probabilistic submodular models, amongst others. DR-submodularity captures a subclass of non-convex functions that enables both exact minimization and approximate maximization in polynomial time. In this work we study the problem of maximizing non-monotone DR-submodular continuous functions under general down-closed convex constraints. We start by investigating geometric properties that underlie such objectives, e.g., a strong relation between (approximately) stationary points and global optimum is proved. These properties are then used to devise two optimization algorithms with provable guarantees. Concretely, we first devise a "two-phase" algorithm with $1/4$ approximation guarantee. This algorithm allows the use of existing methods for finding (approximately) stationary points as a subroutine, thus, harnessing recent progress in non-convex optimization. Then we present a non-monotone Frank-Wolfe variant with $1/e$ approximation guarantee and sublinear convergence rate. Finally, we extend our approach to a broader class of generalized DR-submodular continuous functions, which captures a wider spectrum of applications. Our theoretical findings are validated on synthetic and real-world problem instances.

==> app.tex <==
\section{Minimizing the difference of two submodular continuous functions}\label{sec-diff}

The following ideas need to be verified: 

\begin{enumerate}
	
	\item Any continuous function can be decomposed as: 
	(1) the difference between two submodular continuous functions, and (2) the difference between two convex functions, which one is better for solving the problem? 
	
	
	I think (1) would be easier in terms of (possibly) having some guarantee.    
	
	\item what about the setting when $\X$ is unbounded  and down-closed?  
	 
\end{enumerate}


\subsection{Learning DPPs}

\citet[Chapter 4]{kulesza2013learning}  uses kernel combinations 
to learn the kernel of a DPP. Given a sequence of $n\times n$ symmetric, 
positive semidefinite matrices $\bmL_1, \cdots, \bmL_d$  indexed by the elements 
of $\groundset$, and a sequence of subsets of $S_1, \cdots, S_T$, finding
$\x\in \R^d, \x\geq 0$ to maximize the log-likelihood,  
\begin{flalign}\label{eq_ldpp}
\L(\x) = \sum_{t=1}^{T}\left[ \log\de{\bmL(\x)_{S_t}} - \log\de{\bmL(\x) + \bmI}  \right], \bmL(\x) = \sum_{i=1}^{d}x_i \bmL_i.
\end{flalign}
This problem is conjectured to be NP-Hard  \citep[Conjecture 4.1]{kulesza2013learning}. \cref{eq_ldpp} is in the form of
the difference of \textit{two} submodular continuous functions. 


\Cref{eq_ldpp} can be formulated in two forms:  i) the difference
of two submodular continuous functions; ii) the difference of
two convex functions. 

\subsection{Stochastic setting for learning DPPs}







